Quality Assessment of Super-Resolved Omnidirectional Image Quality Using Tangential Views

Omnidirectional images (ODIs), also known as 360-degree images, enable viewers to explore all directions of a given 360-degree scene from a fixed point. Designing an immersive imaging system with ODI is challenging as such systems require very large resolution coverage of the entire 360 viewing space to provide an enhanced quality of experience (QoE). Despite remarkable progress on single image super-resolution (SISR) methods with deep-learning techniques, no study for quality assessments of super-resolved ODIs exists to analyze the quality of such SISR techniques. This paper proposes an objective, full-reference quality assessment framework which studies quality measurement for ODIs generated by GAN-based and CNN-based SISR methods. The quality assessment framework offers to utilize tangential views to cope with the spherical nature of a given ODIs. The generated tangential views are distortion-free and can be efficiently scaled to high-resolution spherical data for SISR quality measurement. We extensively evaluate two state-of-the-art SISR methods using widely used full-reference SISR quality metrics adapted to our designed framework. In addition, our study reveals that most objective metric show high performance over CNN based SISR, while subjective tests favors GAN-based architectures.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

High-resolution omnidirectional images (ODIs) are quintessential to provide a sufficiently high-quality immersive experience for head-mounted displays. Single image super-resolution (SISR), a fundamentally ill-posed problem, enhances the resolution of a low-resolution image. While no existing consumer cameras can capture very large resolution, such as $\geq$8K, SISR techniques have emerged as a viable option for ODI \cite{360sr}. From traditional hand-crafted approaches to deep learning techniques, SISR methods for ODIs aim to construct the high-resolution ODIs using objective criteria adhering to SISR frameworks for standard images.

ODI processing systems can be optimized by leveraging the techniques of SISR. Similarly to the traditional image, quality assessment plays a vital role. However, no quality assessment framework exists in the literature that can measure and analyze the perceptual efficacy of the super-resolved ODIs while catering to its inherent spherical distortions. Without appropriate quality assessments, the viability of SISR for ODI techniques that promise immersive experience cannot be established.

Many recent learning-based SISR works have achieved remarkable improvements over traditional techniques. Majority of the existing SISR works aim to improve the super-resolved images' accuracy by minimizing the mean squared reconstruction error. With the invention of generative adversarial networks (GANs), state-of-the-art SISR methods claim to achieve higher perceptual quality and better realistic super-resolved images. 

% \ar{should we raise some comment that GANs perform low on metrics normally like in SRGAN?}
While recent SISR works have improved quantitative results, there is an inconsistency between quantitative and qualitative results. Convolutional neural networks (CNNs) and generative adversarial networks (GANs) show great success for SISR. For instance, the super-resolution generative adversarial network (SRGAN)~\cite{ledig2017photo} shows that the high PSNR values do not always accord with better perceptual quality. The reason of this situation is that GAN-based SISR methods often produce realistic yet fake details and textures on the generated super-resolved images \cite{jinjin2020pipal}, bringing a challenge for existing image quality assessment methods.
% \ar{makes sense}

SISR for ODI techniques should produce images with high perceptual quality to have an enhanced immersive viewing experience. However, the lack of understanding of the distortion of super-resolved ODIs motivates us to develop a quality measurement framework, and analyze the distortions of SISR and the performance of quality metrics. In particular, in our previous work \cite{360sr}, we showed that widely used quality metrics (SSIM, PSNR) developed for standard 2D images do not perform well for SISR on ODIs. Hence, we believe that analyzing quality metrics is crucial for designing an optimal SISR method for ODIs. Nevertheless, ODI quality evaluation analysis for SISR was not considered in the literature. To this end, in this study, we target the following objectives: 1) designing a novel SISR quality assessment framework for ODI; 2) performing a thorough evaluation study using state-of-the-art SISR methods for ODIs over state-of-the-art image quality assessment frameworks; 3) investigating the qualitative and quantitative results of CNN- and GAN- based SISR results.

This paper systematically evaluates a broad set of full-reference image quality assessment models with tangential views of ODI. We first developed an objective full-reference ODI quality assessment framework and studied quality measurement for ODIs generated by SISR methods. The proposed quality assessment framework considers the spherical nature of a given ODI with tangential views. These distortion-free tangential views are used to perform a large-scale comparison with eleven perceptual image quality assessment models and state-of-the-art SISR methods for ODI. This study presents the first quality assessment framework to assess the perceptual quality of super-resolved ODIs generated by state-of-the-art SISR methods. Moreover, this is the first evaluation study showcasing the performance of perceptual image quality assessment models on state-of-the-art SISR methods for ODIs. %\co{talk what we found here} 

In this study, we present a straightforward comparison of objective and subjective analysis where we observe that GAN models shows superior performance in subjective tests over conventional CNN SISR architectures. However, contrary to it all the objective metrics favor the CNN models except a few. 


